Shifting Attention to Relevance: Towards the Predictive Uncertainty Quantification of Free-Form Large Language Models

Large Language Models (LLMs) show promising results in language generation and instruction following but frequently "hallucinate", making their outputs less reliable. Despite Uncertainty Quantification's (UQ) potential solutions, implementing it accurately within LLMs is challenging. Our research introduces a simple heuristic: not all tokens in auto-regressive LLM text equally represent the underlying meaning, as "linguistic redundancy" often allows a few keywords to convey the essence of long sentences. However, current methods underestimate this inequality when assessing uncertainty, causing tokens with limited semantics to be equally or excessively weighted in UQ. To correct this, we propose Shifting Attention to more Relevant (SAR) components at both token- and sentence-levels for better UQ. We conduct extensive experiments involving a range of popular "off-the-shelf" LLMs, such as Vicuna, WizardLM, and LLaMA-2-chat, with model sizes extending up to 33B parameters. We evaluate various free-form question-answering tasks, encompassing domains such as reading comprehension, science Q&A, and medical Q&A. Our experimental results, coupled with a comprehensive demographic analysis, demonstrate the superior performance of SAR. The code is available at https://github.com/jinhaoduan/SAR.

==> tables/pretrained_LLMs_wo_sentsim.tex <==
\newcolumntype{?}{!{\vrule width 1pt}}

\begin{table*}
    \centering

    \adjustbox{width=1\textwidth}{
    
        \begin{tabular}{ccccccccc?cccccc} \toprule
          \multirow{2}{*}{\makecell{Models\&\\Datasets}} & \multicolumn{2}{c}{Lexical Similarity} & \multicolumn{2}{c}{Predictive Entropy} & \multicolumn{2}{c}{LN-Pred. Entropy} & \multicolumn{2}{c}{Semantic Entropy} &  \multicolumn{2}{?c}{\textsc{token}{\textit{SAR}}} & \multicolumn{2}{c}{\textsc{gen}{\textit{SAR}}} & 
         \multicolumn{2}{c}{\textit{SAR}}\\
         \cmidrule(lr){2-3} 
         \cmidrule(lr){4-5}
         \cmidrule(lr){6-7}
         \cmidrule(lr){8-9}
         \cmidrule(lr){10-11}
         \cmidrule(lr){12-13}
         \cmidrule(lr){14-15}
          & RL-0.3 & \cellcolor{gray!30} RL-0.5 &  RL-0.3 & \cellcolor{gray!30} RL-0.5 & RL-0.3 & \cellcolor{gray!30} RL-0.5 & RL-0.3 & \cellcolor{gray!30} RL-0.5 & RL-0.3 & \cellcolor{gray!30} RL-0.5 & RL-0.3 & \cellcolor{gray!30} RL-0.5 & RL-0.3 & \cellcolor{gray!30} RL-0.5  \\
         \midrule
         \multicolumn{15}{l}{\textbf{OPT-2.7b} w./ 10 generations are generated for each question} \\
         \midrule
         CoQA & 0.573 & \cellcolor{gray!30} 0.531 & 0.666 & \cellcolor{gray!30} 0.692 & 0.719 & \cellcolor{gray!30} 0.706 & 0.712 & \cellcolor{gray!30} 0.699 & 0.719 & \cellcolor{gray!30} 0.707 & 0.689 & \cellcolor{gray!30} 0.717 & \textbf{0.742} & \cellcolor{gray!30} \textbf{0.735} \\
         \midrule
         \multicolumn{15}{l}{\textbf{OPT-6.7b} w./ 10 generations are generated for each question} \\
         \midrule
         CoQA & 0.588 & \cellcolor{gray!30} 0.542 & 0.671 & \cellcolor{gray!30} 0.696 & 0.745 & \cellcolor{gray!30} 0.723 & 0.741 & \cellcolor{gray!30} 0.717 & 0.746 & \cellcolor{gray!30} 0.724 & 0.696 & \cellcolor{gray!30} 0.722 & \textbf{0.768} & \cellcolor{gray!30} \textbf{0.750} \\
         \midrule
         \multicolumn{15}{l}{\textbf{OPT-13b} w./ 10 generations are generated for each question} \\
         \midrule
         CoQA & 0.588 & \cellcolor{gray!30} 0.545 & 0.666 & \cellcolor{gray!30} 0.695 & 0.750 & \cellcolor{gray!30} 0.727 & 0.751 & \cellcolor{gray!30} 0.726 & 0.752 & \cellcolor{gray!30} 0.729 & 0.690 & \cellcolor{gray!30} 0.720 & \textbf{0.773} & \cellcolor{gray!30} \textbf{0.753} \\
         \midrule
         \multicolumn{15}{l}{\textbf{OPT-30b} w./ 5 generations are generated for each question} \\
         \midrule
         CoQA & 0.550 & \cellcolor{gray!30} 0.505 & 0.671 & \cellcolor{gray!30} 0.696 & 0.742 & \cellcolor{gray!30} 0.719 & 0.751 & \cellcolor{gray!30} 0.726 & 0.746 & \cellcolor{gray!30} 0.723 & 0.698 & \cellcolor{gray!30} 0.723 & \textbf{0.767} & \cellcolor{gray!30} \textbf{0.748} \\
         \midrule
         \multicolumn{15}{l}{\textbf{LLaMA-7b} w./ 5 generations are generated for each question} \\
         \midrule
         CoQA & 0.511 & \cellcolor{gray!30} 0.488 & 0.646 & \cellcolor{gray!30} 0.666 & 0.673 & \cellcolor{gray!30} 0.681 & 0.672 & \cellcolor{gray!30} 0.682 & 0.672 & \cellcolor{gray!30} 0.677 & 0.635 & \cellcolor{gray!30} 0.658 & \textbf{0.686} & \cellcolor{gray!30} \textbf{0.697} \\
         Trivia QA & 0.533 & \cellcolor{gray!30} 0.506 & 0.713 & \cellcolor{gray!30} 0.724 & 0.783 & \cellcolor{gray!30} 0.788 & 0.814 & \cellcolor{gray!30} 0.814 &  0.793 & \cellcolor{gray!30} 0.797 &  0.800 & \cellcolor{gray!30} 0.815 &  \textbf{0.818} & \cellcolor{gray!30} \textbf{0.823} \\
         \midrule
         \multicolumn{15}{l}{\textbf{LLaMA-13b} w./ 5 generations are generated for each question} \\
         \midrule
         CoQA & 0.522 & \cellcolor{gray!30} 0.487 & 0.617 & \cellcolor{gray!30} 0.654 & 0.653 & \cellcolor{gray!30} 0.668 & 0.652 & \cellcolor{gray!30} 0.667 & 0.653 & \cellcolor{gray!30} 0.666 & 0.610 & \cellcolor{gray!30} 0.647 & \textbf{0.665} & \cellcolor{gray!30} \textbf{0.684}  \\
         Trivia QA & 0.655 & \cellcolor{gray!30} 0.616 & 0.492 & \cellcolor{gray!30} 0.488 & 0.627 & \cellcolor{gray!30} 0.606 & \textbf{0.758} & \cellcolor{gray!30} 0.732 & 0.635 & \cellcolor{gray!30} 0.614 & 0.749 & \cellcolor{gray!30} \textbf{0.743} & 0.716 & \cellcolor{gray!30} 0.695 \\
         \midrule
         \textbf{Average} & 0.565 & \cellcolor{gray!30} 0.528 & 0.643 & \cellcolor{gray!30} 0.582 & 0.712 & \cellcolor{gray!30} 0.702 & 0.731 & \cellcolor{gray!30} 0.720 & 0.715 & \cellcolor{gray!30} 0.705 & 0.696 & \cellcolor{gray!30} 0.718 & \textbf{0.742} & \cellcolor{gray!30} \textbf{0.736} \\
         \bottomrule
    \end{tabular}
   
    }
    
    \caption{Uncertainty estimation AUROCs of \textsc{token}{\textit{SAR}}, \textsc{gen}{\textit{SAR}}, \textit{SAR}, and baseline methods, across various ``off-the-shelf'' LLMs and datasets (e.g., CoQA, and Trivia QA). Rouge-L (RL) is used as the correctness metric, with the thresholds set to 0.3 (the default setting in \textit{SE}~\cite{kuhn2023semantic}) and 0.5 (a more harsh correctness standard).}
    \label{tab:main_result}
    \vspace{-2mm}
\end{table*}

==> tables/pretrained_LLMs_wo_sentsim_RL0.5.tex <==


\begin{table*}
    \centering
    \caption{Uncertainty estimation AUROCs of \textsc{token}{\textit{SAR}}, \textsc{gen}{\textit{SAR}}, \textit{SAR}, and baseline methods, across various ``off-the-shelf'' LLMs and datasets (e.g., CoQA, and Trivia QA). Rouge-L with a threshold of 0.5 is used as the correctness metric.\jh{replace with barplot/line plot and move this to appendix}}
    \label{tab:main_result}
\scriptsize
    \adjustbox{width=0.9\textwidth}{
    
        \begin{tabular}{clcccc|ccc} \toprule
        \makecell{Dataset} & Model & \textit{LS} & \textit{PE} & \textit{LN-PE} & \textit{SE} & \textsc{token}{\textit{SAR}} & \textsc{gen}{\textit{SAR}} & \textit{SAR} \\
        \midrule
        \multirow{6}{*}{CoQA} & OPT-2.7b & 0.531 & 0.692 & 0.706 & 0.699 & 0.707 & 0.717 & \textbf{0.735} \\
        & OPT-6.7b &  0.542 &  0.696 &  0.723 &  0.717 &  0.724 &  0.722 &  \textbf{0.750} \\
        & OPT-13b & 0.545 & 0.695 & 0.727 & 0.726 & 0.729 & 0.720 & \textbf{0.753} \\
        & OPT-30b & 0.505 & 0.696 & 0.719 & 0.726 & 0.723 & 0.723 & \textbf{0.748} \\
        \cmidrule{2-9}
        & LLaMA-7b &  0.488 &  0.666 &  0.681 &  0.682 &  0.677 &  0.658 &  \textbf{0.697} \\
        & LLaMA-13b &  0.487 &  0.654 &  0.668 &  0.667 &  0.666 &  0.647 &  \textbf{0.684}  \\
        \midrule
        \multirow{2}{*}{TriviaQA} & LLaMA-7b &  0.506 &  0.724 &  0.788 &  0.814 &  0.797 &  0.815 &  \textbf{0.823} \\
        & LLaMA-13b &  0.616 &  0.488 &  0.606 &  0.732 &  0.614 &  \textbf{0.743} &  0.695 \\
        \midrule
        \multicolumn{2}{c}{\textbf{Average}} & 0.528 &	0.664 & 0.702 &	0.720 &	0.705 &	0.718 &	\textbf{0.736} \\
         \bottomrule
    \end{tabular}
   
    }
    
    
    \vspace{-2mm}
\end{table*}

==> tables/similarity_and_medical.tex <==

\begin{table}[t]
    \begin{minipage}{0.54\textwidth}
    \centering
    \adjustbox{width=\textwidth}{
    \begin{tabular}{cc|ccccc}
        \midrule
        & & \multicolumn{4}{c}{\textit{SAR} w. sentence similarity } \\
         OPT Model Size & \textit{SE} &  RoBERTa & MiniLM & MPNet & OPT-13b \\
          \midrule
        2.7b & 0.699 & \textbf{0.735} & 0.723 & 0.723 & 0.716\\
         6.7b & 0.717 &  \textbf{0.750} &0.740&0.739&0.731 \\
         13b & 0.725 & \textbf{0.753}&0.741&0.740&0.733 \\
         30b & 0.726 & \textbf{0.748}&0.738&0.739&0.734 \\
          \midrule
    \end{tabular}
    }
    \caption{Sensitivity of \textit{SAR} to sentence similarity measurements. We consider two more models from SentenceTransformers (\cref{appendix:sentence_similarity}) and also the target LLMs as the sentence similarity measurement.}
    \label{tab:sentence_similarity}
    \end{minipage}\hfill
    \begin{minipage}{0.45\textwidth}
    \centering
    \adjustbox{width=\textwidth}{
    \begin{tabular}{cc|ccc}
        \midrule
         Model  & Dataset &  \textit{LN-PE} & \textit{SE} & \textit{SAR} \\
          \midrule
        \multirow{2}{*}{Vicuna-13b} & MedQA & 0.572 & \textbf{0.599} & 0.598 \\
         & MedMCQA & 0.649 & 0.685 & \textbf{0.717} \\
        \midrule
        \multirow{2}{*}{LLaMA-2-13b-chat} & MedQA  & 0.562 & 0.609 &\textbf{ 0.616} \\
        & MedMCQA & 0.647 & 0.655 & \textbf{0.702} \\
        \midrule
        WizardLM-13b & MedQA & 0.609 & 0.620 & \textbf{0.635}\\
          \midrule
    \end{tabular}
    }
    \caption{The performance of \textit{SAR} and baseline methods over medical Q\&A datasets. Our method achieves better performances for most settings.}
    \label{tab:medical_results}
    \end{minipage}
    \vspace{-2mm}
\end{table}
